TSpec-LLM: An Open-source Dataset for LLM Understanding of 3GPP Specifications

Understanding telecom standards involves sorting through numerous technical documents, such as those produced by the 3rd Generation Partnership Project (3GPP), which is time-consuming and labor-intensive. While large language models (LLMs) can assist with the extensive 3GPP knowledge base, an inclusive dataset is crucial for their effective pre-training and fine-tuning. In this paper, we introduce \textit{TSpec-LLM}, an open-source comprehensive dataset covering all 3GPP documents from Release 8 to Release 19 (1999--2023). To evaluate its efficacy, we first select a representative sample of 3GPP documents, create corresponding technical questions, and assess the baseline performance of various LLMs. We then incorporate a retrieval-augmented generation (RAG) framework to enhance LLM capabilities by retrieving relevant context from the \textit{TSpec-LLM} dataset. Our evaluation shows that using a naive-RAG framework on \textit{TSpec-LLM} improves the accuracy of GPT-3.5, Gemini 1.0 Pro, and GPT-4 from 44\%, 46\%, and 51\% to 71\%, 75\%, and 72\%, respectively.

==> 02_LLM_background.tex <==
\section{LLMs Functionalities and Limitations}
\label{llm-explained}

Large language models (LLMs) are neural networks primarily based on the transformer architecture, capable of processing extensive sets of unlabeled textual data to comprehend and generate human-like language \cite{vaswani2017attention}. The self-attention mechanism, central to the transformer architecture, is crucial in capturing statistical patterns and relationships within the data, allowing the model to predict and generate information. In this mechanism, each word within an input sequence assesses all other words, computing attention scores that indicate the importance of each word in relation to the rest. This enables the model to capture long-distance correlations and understand how each word is used within its context. Another crucial element in the transformer architecture is multi-head attention, which builds upon the concept of self-attention \cite{wang2020enhancing}. Multi-head attention enhances this by allowing the model to focus on different aspects of the input, capturing diverse patterns and dependencies within the input sequence. This ability helps the model understand complex relationships among words and gain a comprehensive understanding of the input.

LLMs undergo extensive pretraining on large volumes of text data to develop an understanding of the inherent statistical properties of the language. This involves adjusting the model's weights to enable it to forecast the next word in a sentence based on the preceding words. Due to the diverse corpora used in training and the large number of model parameters, LLMs can acquire a thorough grasp of grammar, reasoning capabilities, and even comprehend complex language structures, including foundational wireless communication concepts if included in the pretraining dataset.

\hl{How relevant is this to the paper?}
\red{The primary goal of an LLM is to produce coherent text given a context, but this text might be entirely fabricated, a phenomenon known as hallucination. To enhance an LLM's usability, it undergoes post-processing steps, including supervised fine-tuning and reinforcement learning from human feedback (RLHF) \cite{christiano2017deep}. A small subset of carefully curated data for fine-tuning can significantly improve an LLM's quality \cite{bai2022training}. Fine-tuning guides an LLM to focus on text distributions useful to humans or within specific domains like wireless communication. The RLHF process creates a reward model based on human feedback collected from interactions with models like GPT-4, developed by OpenAI \cite{openai2023gpt4}, and Llama 3 Instruct, developed by Meta \cite{Llama2}. Enhanced through RLHF, a model can generate AI feedback as a substitute for human feedback. However, RLHF is unstable and requires a separate reward model. Direct Preference Optimization (DPO) \cite{rafailov2023direct} addresses these issues by using the LLM itself as the reward model, relying only on user preferences. Iterative improvement through curated instructions (high-quality tokens guiding the model) is another area of research. Algorithms like Self-Play Fine-Tuning (SPIN) aim to align the LLM's output probability distribution with curated datasets \cite{chen2024self-spin}. This approach outperforms DPO after 1-2 iterations, but its performance is limited by the quality of the underlying curated dataset.}

A high-quality dataset combined with recent LLM advancements can improve baseline LLM performance on telecom-specific tasks. The provided open-source TSpec-LLM dataset that we provide aims to close this gap by generating a curated dataset while maintaining the structure of the underlying 3GPP documents (e.g., version, release, etc.).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \rasoul{Zephyr 7B is a model built on top of Mistral 7B V1 \cite{jiang2023mistral} that is capable of utilizing the DPO technique, which is based on syntactic AI feedback. We use this model alongside the newly released open weight model, Mixtral (mixture of expert models by Mistral) \cite{jiang2024mixtral}, to investigate their knowledge in the wireless domain, specifically 3GPP specifications. We chose these models because they provide best-in-class performance for their size and can be modified and fine-tuned for wireless applications, a direction that we will cover in our future work. In addition we heavily utilize the GPT 4 model for question generation ... Finally, we assess GPT 4, GPT 3.5 and Gemeni Pro as additional  proprietary model for performance evaluation.
% }

% \rasoul{As we mentioned, the knowledge of an LLM comes from the pre-training phase. We can enhance model performance by providing more domain-specific information at inference time. We will cover this in the RAG section.}


% \rasoul{Although}

%Although LLMs offer considerable potential, it's essential to acknowledge and understand their limitations to effectively use and interpret the content they generate \cite{bang2023multitask}. 
%The intricate architecture and the vast number of parameters in these models make it challenging to trace their decision-making process, a phenomenon often referred to as limited explainability. LLMs often lack clarity regarding the specific features or patterns they use to generate responses. This lack of transparency hinders the understanding of why a certain answer or response was selected over others. Another drawback is their tendency to produce hallucinations or fabrications. As these models function based on statistical patterns and associations they have learned from extensive text data during training, they might generate responses that imitate these patterns but are factually inaccurate or entirely fictitious. Additionally, LLMs are sensitive to updates and show a pronounced sensitivity to changes in their parameters. This sensitivity hinders their ability to quickly adapt to new trends and recent information. As a result, LLMs may provide responses that are outdated or inaccurate, reflecting their limitations in keeping up with the latest developments and specific domain knowledge. Furthermore, While pretrained LLMs possess a comprehensive and multidisciplinary understanding of the statistical properties within the language they model, they still require domain-specific knowledge for them to be used in industrial applications. To accomplish this, the parameters of the pretrained LLMs undergo fine-tuning using domain-specific datasets and training techniques akin to those employed during the initial pretraining phase. This process, known as knowledge fine-tuning, allows the LLM to adjust the learned representations (embeddings) from the pretraining phase to better align with the particularities  of the specific domain \cite{ding2023parameter}. Addressing the shortcomings outlined, we propose the need for a domain-specific dataset centered on the telecommunications industry, emphasizing standardization and technical specifications. This comprehensive dataset is vital for the pre-training and fine-tuning phases of LLMs to ensure a thorough understanding of the telecom sector. It will serve as a basis for addressing the challenges of applying LLMs to the telecom sector. Additionally, developing a RAG framework using this dataset could help mitigate the issues of limited explainability, hallucinations, and sensitivity to updates.



==> 03_Dataset_Creation.tex <==
\section{TSpec-LLM Dataset Creation}

The dataset contains processed documentation files from the 3GPP standards, converted to markdown (.md) format to facilitate natural language processing applications. It is intended for use by researchers utilizing LLMs, \red{particularly} \hl{ONLY?} those focusing on telecommunications standards.

The documents were downloaded from the 3GPP website \cite{3gpp2024} using the open-source tool download3gpp 0.7.0 \cite{download_3gpp2020}. This tool downloads all documents from all releases and series to a directory. The dataset was then processed using a custom-designed Python script, available open-source\footnote{\href{https://huggingface.co/datasets/rasoul-nikbakht/TSpec-LLM}{https://huggingface.co/datasets/rasoul-nikbakht/TSpec-LLM} \hl{Why not putting it in a reference? It comes up often in the paper.}}. The script utilizes the command-line version of LibreOffice and processes the files in parallel, significantly speeding up the process. This headless conversion process is suitable for server-side operations and batch-processing scripts, resulting in a well-structured and versatile dataset, particularly apt for natural language processing using LLMs in the telecom domain. Unlike the SPEC5G dataset \cite{karim2023spec5g}, which filters out significant content, TSpec-LLM preserves the full content of each document, totaling 535 million words compared to SPEC5G's 134 million words.

%\subsection{Insights to the Dataset}

\begin{comment}
\hl{Isn't this for the conclusions?} \red{As the 3GPP documentation contains many formulas and image captions, future versions of the dataset will use an ML-based processing tool to handle mathematical formulas more efficiently} \footnote{\url{https://github.com/transpect/docx2tex}} \footnote{\url{https://github.com/VikParuchuri/marker}}.
\end{comment}

A Python script was used to analyze the file size of Markdown documents in the \texttt{3GPP-clean} directory. This analysis covered all releases and versions of the 3GPP documentation, calculating the total size of .md files. Results were compiled into a report, categorized by version and release, and saved in JSON format. Fig.~\ref{fig:dataset_tokens} depicts the total size in megabytes for each release, as well as the total word counts (in millions). A visualization of TSpec-LLM is given in Appendix \ref{dataset_vis}.

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/2024_05_21_wordCount_fileSize.eps}
\caption{Word counts (in millions) and file sizes in MB across various 3GPP releases. Data cut off is December 2023.}
\label{fig:dataset_tokens}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{More advanced data processing pipeline}

%The script focuses on the efficient handling and conversion of a large collection of 3GPP documents. The processing followed a two-step parallel approach to manage the high volume of files effectively.

%\subsubsection*{Initial preparation and verification} The script operates within the '3GPP-all' base directory, targeting documents in its sub-directories. The Key functions include 'file exists' for verifying file existence and 'unzip task directory' for automating the unzipping process of the downloaded files. Once the files are retrieved, systematic traversal through nested directory structures is implemented to identify and prepare the files for processing.

%\subsubsection*{Parallel processing for efficiency} Utilized 'ThreadPoolExecutor' for parallel processing, enhances the efficiency of unzipping and document conversion tasks. To address the challenge of converting a large number of documents simultaneously, the script employs multiple LibreOffice instances in parallel. This is achieved by running multiple isolated LibreOffice instances, each with a unique user profile directory.

%\subsubsection*{Document conversion methodology} The script converts the documents to PDF, DOCX, and Markdown formats. For each document, a unique identifier is generated, and a corresponding LibreOffice user profile directory is created. The conversion process is headless, making it suitable for server-side operations and batch-processing scripts.

%\subsubsection*{File size analysis and management} A separate Python script is developed to analyze the file size of Markdown documents in the '3GPP-clean' directory. The script traversed through different releases and versions of the 3GPP documentation, calculating the total size of the .md files. The output is compiled into a comprehensive report, broken down by version and release, and saved as a JSON file. This analysis is believed to be crucial for managing and understanding the distribution of document sizes within the dataset. The total size in megabytes (MB) of each release are represented in Fig.~\ref{fig:dataset_size}, whereas Fig.~\ref{fig:dataset_tokens} shows the number of tokens (in millions) for each release. In the context of LLMs, tokens can be thought of as units of text that the language models process and generate. For English text, a token is approximately 3 characters, which is nearly 0.7 words.

%As a result, the mentioned data processing approach ensured the creation of a well-structured and versatile clean dataset, suitable for various applications, with a special focus on natural language processing by utilizing LLMs for the telecom domain. \blue{It should be noted that different from SPEC5G dataset\cite{karim2023spec5g}, our dataset is comprehensive, well-structured and reserves the full content within every document. In \cite{karim2023spec5g}, the documents undergo a filtering process which removes symbols, unicode characters, tables and the content within them. Such information contained within the tables is considered to be important in the specifications as they consist of system parameters, configurations, and several other technicalities. Moreover, only a specific subset of the entire documents are chosen in \cite{karim2023spec5g}, resulting in a total of 190 million tokens, where as the full 3GPP documents contained in our dataset have a total of 700 million tokens.}
% \rasoul{I think we should keep the one that shows the number of words and only mention the total dataset size in megabits in the text.
% }\mohamed{Sounds good, I agree. I remember you had the raw data for this, can you please send it and I will create a bar graph representation for the manuscript}

% \begin{figure}
% \centering
% \includegraphics[width=\figwidth]{Figures/dataset_size_MB.png}
% \caption{Total size of .md files for each 3GPP release (better quality of the fig. needed and merge it with Fig.2 as 2 sub-plots). .}
% \label{fig:dataset_size}
% \end{figure}

==> 04_benefit.tex <==
\section{How to Benefit from This Dataset}


\hl{I have mixed feelings about this section. Should the title be specific to RAG now? Does the section contain anything novel or just preliminaries? Should it be merged with the next one?} \blue{[Md]: I think we can merge it with the next section}

The TSpec-LLM dataset can be utilized in the context of retrieval-augmented generation (RAG). We provide a detailed application-based explanation to facilitate community adoption of our proposed dataset.

\subsection*{Retrieval-Augmented Generation (RAG):}

\begin{comment}
\red{Although state-of-the-art large language models (LLMs) like the GPT series \cite{brown2020language, openai2023gpt4}, Gemini \cite{team2023gemini}, and others demonstrate remarkable language and knowledge mastery, surpassing human levels in several evaluation benchmarks \cite{srivastava2022beyond}, they still exhibit shortcomings when dealing with specific domains or highly specialized queries \cite{kandpal2023large}. For example, when a user's query extends beyond the model’s pre-training data or requires recent information, LLMs may fail to provide accurate answers. Such limitations pose significant challenges when deploying LLM-based applications in real-world production environments.}
%
\footnote{\hl{This part seems important, but why here and not earlier? We should convince the reader about the need for the dataset once and then move on. I may be wrong, but this sounds like back and forth.} \blue{Md: Done}}
%
\end{comment}

The retrieval-augmented generation (RAG) framework uses an embedding model to assess the similarity among text segments in extensive documents. This model transforms text blocks, limited by a window size of $W$ tokens, into vectors within a $D$-dimensional space, converting textual strings to the mathematical space $\textit{R}^D$. For tasks like responding to telecommunications-related queries, a specialized database like TSpec-LLM can be utilized. This database, potentially encompassing the entirety or selected portions of the 3GPP dataset, is segmented into overlapping or distinct chunks, each smaller than $W$ tokens. These segments are processed offline to generate their respective embeddings.

Several open-source platforms, including LlamaIndex \cite{Liu_LlamaIndex_2022} and LangChain, facilitate this process and are compatible with various embedding models. During the inference phase, the task involves embedding the query prompt and associated metadata to identify the vector in the database that most closely matches the query. The database is typically designed to efficiently retrieve the top K vectors with the highest similarity, along with the corresponding text segments. An example of such a system is Faiss \cite{douze2024faiss}, suitable for handling extensive datasets in the order of billions of words. Faiss operates on both CPU and GPU platforms, efficiently managing vast vector databases and grouping vectors based on similarity.

The RAG framework uses the most pertinent text chunks, identified as the top K similar segments, in conjunction with the original query to accomplish its tasks. This approach strategically places the most relevant information into the working context window of the LLM engaged in the task. Given the LLM's proficiency in exploiting the data within its immediate context, the efficacy of the RAG framework is more likely constrained by the embedding model quality and the LLM's inherent reasoning and retrieval capabilities, rather than by the limitations of the LLM's existing knowledge base. Such a framework is referred to as the naive-RAG paradigm, illustrated in Fig.~\ref{fig:RAG_framework}.

\begin{figure}
\centering
\includegraphics[width=.99\figwidth]{Figures/RAG framework.png}
\caption{Naive-RAG paradigm}
\label{fig:RAG_framework}
\end{figure}

In the context of telecom knowledge, we can deploy a RAG framework on top of each release, utilizing a strong open-source model to add annotations to each document and each chunk to increase the likelihood of finding the best match. Additionally, a separate model can augment the query to the RAG framework, effectively increasing the potential overlap between the given text or question and the desired chunk of text from standardization.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\rasoul{New}:The RAG framework relies on an embedding model to determine the similarity between different chunks of text in long documents. In essence, an embedding model converts chunks of text with a maximum window size of $W$ tokens into $D$-dimensional real vectors, effectively mapping from a string to $\textit{R}^D$. For a given task, in this case, answering telecom-related questions, we can create a database of domain knowledge or any other information we think is useful for the task,e.g., the whole or a subset of the curated 3GPP dataset, and divide them into overlapping or non-overlapping chunks of $C<W$. Then, in an offline manner, we compute the embedding for all the chunks in our database. There are several open-source tools that handle this step, including LlamaIndex and LangChain. These tools can work with a variety of embedding models. At inference time, when performing the task, we embed the query prompt alongside other metadata and try to find the most similar vector in our vector database. Typically, the vector database implements an efficient search algorithm for retrieving the top K similar vectors, and consequently, text chunks. For instance, Faiss, a nearest-neighbor search implementation for billion-scale datasets, which works on both CPU and GPU, can handle a large vector database and cluster similar vectors.

\begin{comment}
\subsection{Fine-tuning a base model}
As we outlined in section \ref{llm-explained}, the quality of the dataset plays a crucial role in enhancing the performance of a model for a specific task (telecom-specific understanding). The provided dataset (3GG-for-LLM) can be utilized to create a telecom-specific fine-tuning dataset using other high-performing models. This approach has been explored in depth for various open-source models such as the Wizard LLM \footnote{\url{https://huggingface.co/WizardLM}} \cite{xu2023wizardlm} and the Phi model family \cite{abdin2024phi3,gunasekar2023textbooks}, yielding excellent results. 

The Phi model family approach is based on designing a detailed data curation framework for the given task and producing synthetic data using a stronger model (teacher model). In the case of telecom knowledge, we already have a significant head start since the expert knowledge is well documented by the standardization bodies, which is reflected in our proposed dataset. We can set up a framework where most or all of the documents are systematically fed into a strong base model, then ask it to provide annotations and instructions for each chunk of text. Using this extra curated dataset, we can fine-tune open-source base models such as Llama-3 8B or Phi3, and provide a strong telecom model that can also be utilized in an offline fashion using tools such as Ollama\footnote{\url{https://github.com/ollama/ollama}}.
\end{comment}




%To adapt to a specific domain or proprietary information, the base model of an LLM undergoes fine-tuning to parameterize knowledge. While this method yields to enhancing the model results accuracy, it demands substantial computational resources and requires high costs. Both parametric and non-parametric knowledge play distinct roles. Parametric knowledge represents the model’s understanding and generalization of the training data, stored in the neural network weights, forming the foundation for the generated responses. On the other hand, non-parametric knowledge resides as external sources; i.e., vector databases, which are not encoded directly into the base model, rather treated as supplementary information. This non-parametric knowledge empowers LLMs to process and learn the latest domain specific information; thus, enhancing the accuracy and relevance of responses. To address the limitations of purely parameterized models, LLMs can adopt a semi-parameterized approach by integrating a domain specific corpus database to the parameterized base model. This approach is known as Retrieval Augmented Generation (RAG).  The RAG framework allows developers to avoid the need for retraining the LLM for each specific task. Instead, they can attach an external knowledge database, providing additional information input to the model and improving the accuracy of its responses. 

%The term Retrieval-Augmented Generation (RAG) was first introduced in \cite{lewis2020retrieval}, in which a pre-trained retriever is combined with a pre-trained seq2seq model (generator) and undergoes end-to-end fine-tuning to capture knowledge in an explicable and modular way. The RAG framework consists of two key stages; first, utilizing encoding models to retrieve relevant documents based on the query; second, the generation phase, which uses the retrieved context as a condition for the LLM to generate response.

%In this study, we will concentrate on the naive-RAG frameworks. The naive-RAG research approach emerged as a prominent methodology shortly after the widespread adoption of ChatGPT \cite{ma2023query}. The naive-RAG involves: indexing, retrieval, and generation, also known as a “Retrieve”-“Read” framework. The naive-RAG paradigm is illustrated in Fig.~\ref{fig:RAG_framework}. The main attributes of the framework are as follow: 

%\textbf{Indexing}: The pipeline for obtaining information from the source dataset and building an index for it generally occurs in an offline state. Specifically, the construction of a data index involves data indexing, chunking, and embedding.\\
%\textit{Data indexing} is the process of extracting and cleaning the original data, by converting the file formats such as Markdown into plain text. \\
%\textit{Chunking} involves dividing the loaded text into smaller portions, referred to as chunks. This is necessary as LLMs typically have a limit on the amount of context they can handle. \\
%\textit{Embedding} is the process of encoding the text within the chunks into vectors via an LLM. The resulting vectors will be used in the subsequent retrieval process to measure their similarity to the query vector entered by the user. An embedding, is a numerical representation of the semantics of the text. Two pieces of text having similar meanings will have mathematically similar embeddings, even if the actual text is quite different. This mathematical relationship enables semantic search, rather than simple keyword matching.

%\textbf{Retrieve:} Given a user’s query, the same encoding model used in the indexing stage is used again to convert the query into a vector. The similarity between the query embedding and the embedding of the document chunks in the corpus is calculated. The top $k$ document chunks are retrieved based on the level of similarity.

%\textbf{Generation:} The given query and the retrieved $k$ document chunks are combined into a new prompt. The LLM is then tasked to answer the query based on the provided information. The developer can decide whether to allow the model to use its base knowledge or only to answer based on the retrieved information, depending on the needs of the task. 

% \rasoul{To do}: Add a paragraph about the various embedding models, such as Mistral and OpenAI. Explain that there are also open-source options (name a few). Create a simple toy example to illustrate the concept of embedding. Discuss hierarchical embedding as a solution for efficiently managing the full-scale 3GPP clean dataset embedding.





% \rasoul{To do}:The framework should be modified to reflect the components we have used not a general framework. The framework should be modified to accurately reflect the specific components we have utilized, rather than representing a general framework. \mohamed{Can you please sketch what you have in mind on a paper and I will create a figure out from it.}
% \rasoul{We are utilizing llamindex, Mistral embedding,   }



